Spitzer Variability Properties of Low-Gravity L Dwarfs

We present \textit{Spitzer Space Telescope} variability monitoring observations of three low-gravity L dwarfs with previous detections of variability in the near-IR, 2MASS J0045+16, 2MASS J0501-00 and 2MASS J1425-36. We detect significant, periodic variability in two of our targets, 2MASS J0045+16 and 2MASS J0501-00. We do not detect variability in 2MASS J1425-36. Combining our new rotation periods with rotational velocities, we calculate inclination angles of $22\pm1^{\circ}$, ${60^{+13 }_{-8}} ^{\circ}$ and $52^{+19}_{-13}~^{\circ}$ for 2MASS J0045+16, 2MASS J0501-00 and 2MASS J1425-36 respectively. Our three new objects are consistent with the tentative relations between inclination, amplitude and color anomaly previously reported. Objects with the highest variability amplitudes are inclined equator-on, while the maximum observed amplitude decreases as the inclination angle decreases. We also find a correlation between the inclination angle and $(J-K)_{\mathrm{2MASS}}$ color anomaly for the sample of objects with measured inclinations. Compiling the entire sample of brown dwarfs with \textit{Spitzer} variability detections, we find no enhancement in amplitude for young, early-L dwarfs compared to the field dwarf population. We find a possible enhancement in amplitude of low-gravity late-L dwarfs at $4.5~\mu$m. We do not find a correlation between amplitude ratio and spectral type for field dwarfs or for the young population. Finally, we compile the rotation periods of a large sample of brown dwarfs with ages 1 Myr to 1 Gyr and compare the rotation rates predicted by evolutionary models assuming angular momentum conservation. We find that the rotation rates of the current sample of brown dwarfs fall within the expected range set by evolutionary models and breakup limits.

==> Spitzer PID 14019_revision2_arxiv/objects.tex <==
% Awesome system for defining object shorthands. First:
%
% \DefineObj[short name]{nickname}{long name}
%
% Then
%
% \obj*{nickname} => long name
% \obj{nickname} => short name if defined, otherwise long name
%
% The nicknames can include numbers, which is nice because LaTeX command names
% can't!

\makeatletter
\newcommand\DefineObj[3][\@empty]{%
  \expandafter\newcommand\csname pkgwobj@l#2\endcsname{#3}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#3}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%
\newcommand{\pkgw@printobj@long}[1]{%
  \expandafter\ifx\csname pkgwobj@l#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@l#1\endcsname%
  \fi}%
\newcommand{\pkgw@printobj@short}[1]{%
  \expandafter\ifx\csname pkgwobj@l#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@s#1\endcsname%
  \fi}%
\newcommand{\obj}{\@ifstar{\pkgw@printobj@long}{\pkgw@printobj@short}}%
\makeatother

==> Spitzer PID 14019_revision2_arxiv/spts.tex <==
\startlongtable
\begin{longrotatetable}
\begin{deluxetable}{lcccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{12}
\tablenum{3}
\tablewidth{0pt}
\setlength{\tabcolsep}{0.05in}
\tablecaption{Brown dwarf variability detections and upper limits in the infrared \label{tab:variables}}
\tablehead{  
%\cline{4-8}
%\cline{9-11}
%\colhead{Designation} & 
%\colhead{Adopted} &  
\colhead{Target} &
\colhead{SpT} & 
\colhead{$A_{J}$} & 
\colhead{$A_{3.6}$} & 
\colhead{ $A_{4.5}$} & 
\colhead{Period } & 
\colhead{Age } & 
\colhead{Radius$^\mathrm{a}$} & 
\colhead{Companion} & 
\colhead{Inclination } & 
\colhead{Variability} \\
\colhead{} &
\colhead{} & 
\colhead{(\%)  } & 
\colhead{(\%) } & 
\colhead{(\%)} & 
\colhead{(hr)} & 
\colhead{(Myr)} & 
\colhead{($R_{\mathrm{Jup}}$)} & 
\colhead{} & 
\colhead{$(^{\circ})$} & 
\colhead{References}}
\startdata
%\cutinhead{\emph{Bona fide sample}}
2MASS J00132229-1143006	  &T2 (T3.5+T4.5?)	&$4.6\pm0.2$	&\nodata        &\nodata&	        $>2.8$             &	1000       &\nodata             &	0	        &\nodata                    &	1           \\
 LSPM J0036+1821          & L3.5         & $1.22\pm0.04$   & $0.47\pm0.05$   & $0.19\pm0.04$   & $2.7\pm0.3$          & 1000      & $1.01\pm0.07$       & 0   & $51\pm9$                       & 2,3,4        \\
2MASS J00452143+1634446   & L2      & $1.0\pm0.1$           & $0.18\pm0.04$   & $0.16\pm0.04$   & $2.4\pm0.1$          & 50        & $1.62\pm0.06$      & 0         & $23\pm1$            & 5,6         \\
2MASS J00470038+6803543   & L9        & 8                   & $1.07\pm0.04$   &                 & $16.4\pm0.2$        & $130\pm20$ & $1.28\pm0.02^8$      & 0         & $85^{+5}_{-9}$        & 7,4,8       \\
2MASS J00501994-3322402   & T7           & \nodata          & \textless{}0.59 & $1.07\pm0.11$   & $1.55\pm0.02$        & 1000       & $0.94\pm0.16$     & 0         & \nodata                  & 2            \\
2MASSI J0103320+193536    & L6          & \nodata         & $0.56\pm0.03$   & $0.87\pm0.09$     & $2.7\pm0.1$          & $300\pm200$ & $1.34\pm0.13$    & 0         & $40\pm8$               & 2            \\
2MASS J01075242+0041563   & L8           & \nodata          & $1.27\pm0.13$   & $1\pm0.2$       & $5\pm2$              & 1000        & $0.98\pm0.11$    & 0         & $56\pm17$               & 2            \\
GU PSC B                  & T3.5         & $4\pm1$         &  \nodata       &   \nodata         &  \nodata             & $130\pm20$  & \nodata          & 1         & \nodata                 & 9            \\
SIMP J013656.57+093347.3  & T2.5         & 4.5             & $1.5\pm0.2$     &  \nodata         & $2.414\pm0.078$     & $200\pm50$   & $1.22\pm0.01^12$    & 0         & $80\pm12$               & 10,11,12,13,4 \\
2MASS J01383648-0322181	  &T3	          &$5.5\pm1.2$	   &\nodata      	&\nodata	        &\nodata		       &1000	     &\nodata           &0	        &\nodata	               &2               \\
SDSS J015141.69+124429.6  & T0.0         & \nodata        & \textless{}0.83 & \textless{}0.81   & \nodata               & 1000       & $0.97\pm0.16$    & 0         & \nodata               & 2            \\
2MASSW J0310599+164816    & L8          &  \nodata         & \nodata         & \nodata           &   \nodata              & 1000     &\nodata          & 0         &  \nodata               & 14           \\
SDSS J042348.57-041403.5  & L6.5+T2      & $0.8\pm0.08$    &  \nodata          &  \nodata          & $2\pm0.4$            & 1000     &\nodata         & 0         & $79^{+11}_{-16}$          & 15,4         \\
PSO J071.8769-12.2713	  &T2	        &$4.5\pm0.6$	    &\nodata	        &\nodata	       &\nodata	        	&\nodata	 &\nodata           &0	        &\nodata	                &6      \\
2MASS J05012406-0010452   & L4           & $2\pm1$         & $0.36\pm0.04$   & $0.24\pm0.04$        & $15.7\pm0.2$    & $300\pm200$  & $1.38\pm0.18$    & 0         & $73^{+17}_{-12}$         & 5,6          \\
2MASS J05591914-1404488   & T4.5         & $0.7\pm0.5$     &   \nodata         & \nodata           & $10\pm3$           & 1000       & $0.97\pm0.11$      & 0         & \nodata                 & 10            \\
2MASS J06244595-4521548   & L6.5         & \textgreater{}1 &  \nodata          &  \nodata           &                    & 1000      & $0.99\pm0.10$    & 0         & \nodata                & 14           \\
SDSS J075840.33+324723.4  & T0.0+T3.5    & $4.8\pm0.2$     &  \nodata         &   \nodata         & $4.9\pm0.2$          & 1000      &\nodata           & 0         &  \nodata              & 10            \\
DENIS J081730.0-615520    & T6           & $0.6\pm0.1$     & \nodata          &  \nodata         & $2.8\pm0.2$          & 1000       & $0.94\pm0.16$    & 0         &  \nodata             & 10            \\
2MASSW J0820299+450031    & L5          &  \nodata        & \textless{}0.4  & \textless{}0.48       & \nodata               & 1000   &\nodata           & 0         &  \nodata        & 2            \\
2MASSI J0825196+211552    & L7.5        & \textgreater{}1 & $0.81\pm0.08$   & $1.4\pm0.3$           & $7.6\pm5$            & 1000    & $0.98\pm0.11$      & 0         &   \nodata       & 2            \\
SDSS J085834.42+325627.7  & T1           &  \nodata        & \textless{}0.27 & \textless{}0.64  &   \nodata             & 1000       &\nodata            & 0         &  \nodata           & 2            \\
2MASS J09490860-1545485   & T1.0+T2.0    & \nodata         & \textless{}0.54 & \textless{}0.83  &   \nodata            & 1000        & $0.96\pm0.17$     & 0         &   \nodata           & 2            \\
LP261-75B                 & L6V          & $2.4\pm0.14$    &   \nodata       & \nodata          & $4.78\pm0.98$       & $30\pm50$    &\nodata           & 1         &    \nodata            & 16           \\
2MASS J10101480-0406499	  &L6	        &$3.6\pm0.4$	    &\nodata	    &\nodata        	&\nodata	            &1000	     & $0.94\pm0.16$     &0	            &\nodata	        &11             \\
SDSS J104335.08+121314.1  & L9           &  \nodata        & $1.54\pm0.15$   & $1.2\pm0.2$      & $3.8\pm0.2$          & 1000        & $0.98\pm0.11$     & 0         &   \nodata           & 2            \\
WISE 1049B                & L7.5         &   \nodata       &  \nodata        & \nodata          & $4.87\pm0.01$        & 1000        & $1.02\pm0.07$     & 0         & $83^{+7}_{-8}$      & 17,18,4      \\
SDSS J105213.51+442255.7  & L6.5+T1.5    & $2.2\pm0.5$     & \nodata            &  \nodata         & $3\pm0.5$            & 1000     & \nodata           & 0         &  \nodata              & 19           \\
DENIS-P J1058.7-1548      & L2.5         & $0.8\pm0.1$ & $0.39\pm0.04$   & \textless{}0.3       & $4.1\pm0.2$          & 1000        & $1.00\pm0.07$     & 0         & $90^{+0}_{-2}$       & 20,2,4       \\
2MASS J10595185+3042059   & T8           &    \nodata       & \textless{}0.83 & \textless{}0.89 &    \nodata             & 1000      & \nodata           & 0         &  \nodata              & 2            \\
SDSS J111009.99+011613.0  & T5.5         & \nodata         &  \nodata       & \textless{}1.25 &  \nodata              & $130\pm20$   & $1.24\pm0.04$      & 0         & \nodata              & 8            \\
2MASS J11193254-1137466AB & L7           & \nodata          & $0.46\pm0.036$  & $0.96\pm0.037$  & $3.02\pm0.04$        & $7\pm2.5$   & \nodata            & 0         &  \nodata             & 21           \\
2MASS J11220826-3512363   & T2           &  \nodata        & \textless{}0.24 & \textless{}0.31 &                      & 1000         & \nodata            & 0         &  \nodata             & 2            \\
2MASS J11263991-5003550   & L5           & $1.2\pm0.1$     & $0.21\pm0.04$   & $0.29\pm0.15$   & $3.2\pm0.3$          & 1000         & \nodata            & 0         & $35\pm7$             & 10,2,4        \\
WISEA J114724.10-204021.3 & L7          &  \nodata         & $1.596\pm0.08$  & $2.216\pm0.09$  & $19.39\pm0.3$        & $7\pm2.5$    & \nodata          & 0         &   \nodata             & 21           \\
SDSS J115013.17+052012.3  & L6           &  \nodata          & \textless{}0.38 & \textless{}0.65 &                      & 1000       & \nodata            & 0         &  \nodata             & 2            \\
2M1207b                   & L6           & $2.72\pm0.1$            &  \nodata         &  \nodata         & $10.7\pm1$  & $7\pm2.5$   & $1.36\pm0.02$        & 1         &  \nodata        & 22           \\
2MASS J12095613-1004008   & T2+T7.5      &  \nodata         & \textless{}0.4  & \textless{}0.56 &  \nodata               & 1000      & \nodata          & 0         & \nodata               & 2            \\
2MASS J12195156+3128497   & L9           & \textgreater{}2 &   \nodata       & \nodata     &  \nodata              & 1000            & \nodata        & 0         & \nodata                 & 14           \\
SDSS J125453.90-012247.5  & T2         &    \nodata       & \textless{}0.15 & \textless{}0.3  &\nodata             & 1000            & $0.98\pm0.15$         & 0         & \nodata          & 2            \\
VHS1256-1257b             & L7         &    $24.7$       & \nodata           & $5.76\pm0.04$  &$22.04\pm0.05$      & 150-300         & \nodata            & 1         & $90^{+0}_{-29}$     & 23, 24            \\
Ross 458C                 & T8.5        & $2.62\pm0.02$   & \textless{}1.37 & \textless{}0.72 & $6.75\pm1.58$        & $125\pm75$    &\nodata         & 1         &   \nodata               & 25,2         \\
2MASS J13243559+6358284   & T2       &  \nodata         & $3.05\pm0.15$   & $3\pm0.3$       & $13\pm1$             & $130\pm20$      & \nodata       & 0         &\nodata                    & 2            \\
WISE J140518.39+553421.3  & Y0     &    \nodata        & $7.2\pm0.8$     & $7.1\pm0.2$   & $8.2\pm0.3$         & 1000                & \nodata     & 0         &   \nodata                 & 26           \\
ULAS J141623.94+134836.3  & T7.5        &   \nodata        & \textless{}0.91 & \textless{}0.59 &  \nodata              & 1000        & $0.96\pm0.16$         & 0         &  \nodata              & 2            \\
SDSS J141624.08+134826.7  & L6   &   \nodata        & \textless{}0.15 & \textless{}0.22 &   \nodata             & 1000               & \nodata      & 0         &  \nodata              & 2            \\
2MASS J14252798-3650229   & L4           & $0.7\pm0.3$     & \textless{}0.16 & \textless{}0.18 &  \nodata              & $130\pm20$  & $1.32\pm0.09$           & 0         & $52^{+19}_{-13}$      & 5,6          \\
2MASSW J1507476-162738    & L5          & 0.7             & $0.53\pm0.11$   & $0.45\pm0.09$   & $2.5\pm0.1$          & 1000          & $0.99\pm0.09$           & 0         & $23\pm2$              & 11,2,4       \\
SDSS J151114.66+060742.9  & L5.5+T5.0    &   \nodata        & $0.67\pm0.07$   & \textless{}0.49 & $11\pm2$             & 1000        & \nodata           & 0         & \nodata               & 2            \\
SDSS J151643.01+305344.4  & L8.0+L9.5    &  \nodata         & $2.4\pm0.2$     & $3.1\pm1.6$     & $6.7\pm5$            & 1000        & \nodata           & 0         &  \nodata              & 2            \\
SDSS J152039.82+354619.8  & T0           &  \nodata        & \textless{}0.3  & \textless{}0.45 &                      & 1000         & \nodata           & 0         &   \nodata             & 2            \\
SDSS J154508.93+355527.3  & L7.5         &   \nodata        & \textless{}0.59 & \textless{}1.15 &                     & 1000         & \nodata           & 0         &  \nodata              & 2           \\
2MASS J16154255+4953211   & L4           &   \nodata       & $0.9\pm0.2$     & \textless{}0.39 & $24\pm5$             & $300\pm200$  & $0.94\pm0.16$    & 0         & $86^{+4}_{-10}$       & 2,4          \\
2MASS J16291840+0335371   & T2           & $4.3\pm2.4$     & \nodata        &  \nodata    & $6.9\pm2.4$          & 1000              & \nodata            & 0         & $82^{+8}_{-12}$       & 10,4          \\
2MASSW J1632291+190441    & L8           &  \nodata         & $0.42\pm0.08$   & $0.5\pm0.3$     & $3.9\pm0.2$          & 1000        & $0.97\pm0.12$    & 0         &  \nodata              & 2            \\
2MASSI J1721039+334415    & L5.3       &    \nodata      & $0.33\pm0.07$   & \textless{}0.29 & $2.6\pm0.1$          & 1000           & \nodata            & 0         & $27\pm4$              & 2,4          \\
2MASSI J1726000+153819    & L2          &     \nodata      & \textless{}0.29 & \textless{}0.49 &                      & $300\pm200$  & $1.40\pm0.20$        & 0         &  \nodata              & 2            \\
WISEP J173835.52+273258.9 & Y0           &       \nodata   &    \nodata       & $3\pm0.1$       & $6\pm0.1$            & 1000        & \nodata            & 0         &   \nodata             & 27           \\
2MASS J17502484-0016151   & L5           & \textgreater{}1 &   \nodata       &  \nodata         &  \nodata               & 1000      & \nodata           & 0         & \nodata                & 14           \\
2MASS J17503293+1759042   & T3.5         & \textgreater{}1 &   \nodata      &   \nodata          & \nodata                & 1000     & $0.97\pm0.16$      & 0         &  \nodata              & 14           \\
2MASS J17534518-6559559   & L4           &    \nodata       & \textless{}0.25 &   \nodata       &   \nodata            & 1000        & \nodata           & 0         &   \nodata             & 2            \\
2MASS J18212815+1414010   & L5           &  \nodata         & $0.54\pm0.05$   & $0.71\pm0.14$   & $4.2\pm0.1$         & 1000         & \nodata           & 0         & $61\pm17$             & 11,2,4       \\
2MASS J18283572-4849046   & T5.5         & $0.9\pm0.1$     & \nodata          & \nodata           & $5\pm0.6$            & 1000      & $0.95\pm0.16$      & 0         & \nodata               & 10            \\
2MASS J20025073-0521524   & L5.5         & $1.7\pm0.2$     & \nodata           & \nodata           & \nodata        & $300\pm200$    & \nodata              & 0         & \nodata               & 5            \\
SDSS J204317.69-155103.4  & L9.5         & \nodata          & \textless{}0.71 & \textless{}0.74 &  \nodata             & 1000        & \nodata            & 0         & \nodata              & 2            \\
SDSS J205235.31-160929.8  & T1+T2.5 &                 & \textless{}0.36 & \textless{}0.71       &  \nodata            & 1000         & \nodata             & 0         &    \nodata          & 2            \\
PSO 318.5-22              & L7           & $10\pm1.3$      &                 & $3.4\pm0.08$    & $8.61\pm0.06$        & $23\pm3$     & $1.41\pm0.03$       & 0         & $56\pm8$             & 28,29,5      \\
2MASS J21392676+0220226   & L8.5+T3.5    & $26\pm1$            & $11\pm1$        & $10\pm1$        & $7.618\pm0.18$       & 1000     & $0.96\pm0.16$       & 0         & $90^{+0}_{-1}$        & 10,13,4,11    \\
HN PegB                   & T2.5         & 1.2             & $0.77\pm0.15$   & $1.1\pm0.5$     & $15.4\pm0.5$         & $237\pm33$   & \nodata          & 1         &   \nodata              & 2            \\
2MASS J21481628+4003593   & L7           & \nodata         & $1.33\pm0.07$   & $1.03\pm0.1$    & $19\pm4$             & $200\pm200$  & $0.99\pm0.10$           & 0         & $88^{+2}_{-8}$         & 2,4          \\
2MASSW J2208136+292121    & L2      &     \nodata      & $0.69\pm0.07$   & $0.54\pm0.11$   & $3.5\pm0.2$          & $23\pm3$         & $1.41\pm0.20$           & 0         & $55\pm10$             & 2,4          \\
2MASS J22153705+2110554	  &T1 (T0+T2?)	&$10.7\pm0.4$	&\nodata	        &\nodata	    &\nodata	        	&1000	         & \nodata           &0	        &\nodata	             &2               \\
2MASSW J2224438-015852    & L4.5V        &  \nodata      & \textless{}0.1  & \textless{}0.15 &                      & 1000           & $0.99\pm0.08$           & 0         &  \nodata              & 2            \\
2MASS J22282889-4310262   & T6.5         & 5.3             & $4.6\pm0.2$     & $1.51\pm0.15$   & $1.41\pm0.01$        & 1000         & $0.94\pm0.16$            & 0         &  \nodata               & 10,2,30       \\
2MASS J22393718+1617127	  &T3	        &$5.8\pm0.4$	&\nodata	    &\nodata	        &\nodata	        	&1000	         & \nodata           &0	        &\nodata	             &2              \\
2MASS J2244316+204343     & L6-L8   & $5.5\pm0.6$     & $0.8\pm$        &  \nodata          & $11\pm2$             & 120             & $1.28\pm0.02^8$           & 0         & $76^{+14}_{-20}$       & 31,8,5       \\
SDSSp J224953.45+004404.2 & L3+L5        &   \nodata       & \textless{}0.25 & \textless{}0.45 &  \nodata               & 1000       & \nodata             & 0         &  \nodata             & 2            \\
2MASSI J2254188+312349    & T5.0         &  \nodata      & \textless{}0.47 & \textless{}0.39 &   \nodata            & 1000           & \nodata             & 0         &   \nodata               & 2            \\
WISE J085510.83-071442.5  & Y2           &  \nodata         & $4\pm1$         & $4\pm1$         &   \nodata            & 1000        & \nodata              & 0         &  \nodata                & 32           \\
HD 203030B                & L7.5         & $1.1\pm0.3$     &   \nodata       &  \nodata          & $7.5\pm0.6$          & $9\pm60$   & \nodata             & 1         &  \nodata                 & 33      \\ 
\enddata
\tablecomments{Table available online. \\
a. Estimated radii are from \citet{Filippazzo2015}, except where a superscript indicates reference}
\tablerefs{
~(1)~\citet{Eriksson2019};
~(2)~\citet{Metchev2015a};
~(3)~\citet{Croll2016};
~(4)~\citet{Vos2017};
~(5)~\citet{Vos2019};
~(6)~This work;
~(7)~\citet{Lew2016};
~(8)~\citet{Vos2018};
~(9)~\citet{Naud2017};
~(10)~\citet{Radigan2014};
~(11)~\citet{Yang2016};
~(12)~\citet{Gagne2017};
~(13)~\citet{Apai2017};
~(14)~\citet{Buenzli2014};
~(15)~\citet{Clarke2008};
~(16)~\citet{Manjavacas2018};
~(17)~\citet{Gillon2013};
~(18)~\citet{Buenzli2015a};
~(19)~\citet{Girardin2013};
~(20)~\citet{Heinze2014};
~(21)~\citet{Schneider2018};
~(22)~\citet{Zhou2016};
~(23)~\citet{Bowler2020};
~(24)~\citet{Zhou2020};
~(25)~\citet{Manjavacas2019};
~(26)~\citet{Cushing2016};
~(27)~\citet{Leggett2016};
~(28)~\citet{Allers2016};
~(29)~\citet{Biller2018};
~(30)~\citet{Buenzli2012};
~(31)~\citet{Morales-Calderon2006};
~(32)~\citet{Esplin2016};
~(33)~\citet{Miles-Paez2019}}
\end{deluxetable}
\end{longrotatetable}
\clearpage


